Provable Robustness Against a Union of $\ell_0$ Adversarial Attacks

Sparse or $\ell_0$ adversarial attacks arbitrarily perturb an unknown subset of the features. $\ell_0$ robustness analysis is particularly well-suited for heterogeneous (tabular) data where features have different types or scales. State-of-the-art $\ell_0$ certified defenses are based on randomized smoothing and apply to evasion attacks only. This paper proposes feature partition aggregation (FPA) -- a certified defense against the union of $\ell_0$ evasion, backdoor, and poisoning attacks. FPA generates its stronger robustness guarantees via an ensemble whose submodels are trained on disjoint feature sets. Compared to state-of-the-art $\ell_0$ defenses, FPA is up to 3,000${\times}$ faster and provides larger median robustness guarantees (e.g., median certificates of 13 pixels over 10 for CIFAR10, 12 pixels over 10 for MNIST, 4 features over 1 for Weather, and 3 features over 1 for Ames), meaning FPA provides the additional dimensions of robustness essentially for free.

==> tables/med-robust/detailed/ours/ames.tex <==
    & \DetailAccHead{}         & \OursMedRobustHead{}        & \DetailAccHead{}       & \OursMedRobustHead{}     \\\midrule
1   & \DetailAccMed{88.05}     & \DetailMed{0}               & \DetailAccMed{89.25}   & \DetailMed{0}     \\\DetailRaMedKeepSep
5   & \DetailAccMed{84.64}     & \DetailMed{1}               & \DetailAccMed{82.08}   & \DetailMed{1}     \\\DetailRaMedKeepSep
11  & \DetailAccMed{78.50}     & \DetailMed{2}               & \DetailAccMed{74.40}   & \DetailMed{1}     \\\DetailRaMedKeepSep
15  & \DetailAccMed{73.04}     & \DetailMed{2}               & \DetailAccMedB{66.55}  & \DetailMedB{2}     \\\DetailRaMedKeepSep
21  & \DetailAccMedTop{65.53}  & \DetailMedTop{3}            & \DetailAccMed{61.60}   & \DetailMed{2}     \\\DetailRaMedKeepSep
25  & \DetailAccMed{61.77}     & \DetailMed{2}               & \DetailAccMed{57.34}   & \DetailMed{1}     \\\DetailRaMedKeepSep
31  & \DetailAccMed{57.68}     & \DetailMed{2}               & \DetailAccMed{53.58}   & \DetailMed{0}     \\\DetailRaMedKeepSep
35  & \DetailAccMed{55.97}     & \DetailMed{1}               & \DetailAccMed{50.34}   & \DetailMed{0}     \\\DetailRaMedKeepSep
41  & \DetailAccMed{52.90}     & \DetailMed{1}               & \DetailAccMed{46.42}   & \DetailMed{\DetailedNeg{}}     \\\DetailRaMedKeepSep
51  & \DetailAccMed{47.10}     & \DetailMed{\DetailedNeg{}}  & \DetailAccMed{40.10}   & \DetailMed{\DetailedNeg{}}     \\\DetailRaMedKeepSep
75  & \DetailAccMed{36.86}     & \DetailMed{\DetailedNeg{}}  & \DetailAccMed{35.15}   & \DetailMed{\DetailedNeg{}}     \\


==> tables/med-robust/detailed/ours/cifar10.tex <==
     & \DetailAccHead{}       & \OursMedRobustHead{}  & \DetailAccHead{}         & \OursMedRobustHead{}     \\\midrule
5    & \DetailAccMed{91.46}   & \DetailMed{2}         & \DetailAccMed{91.77}     & \DetailMed{2}     \\\DetailRaMedKeepSep
10   & \DetailAccMed{86.09}   & \DetailMed{4}         & \DetailAccMed{86.20}     & \DetailMed{4}     \\\DetailRaMedKeepSep
20   & \DetailAccMed{81.38}   & \DetailMed{7}         & \DetailAccMed{81.40}     & \DetailMed{7}     \\\DetailRaMedKeepSep
25   & \DetailAccMed{78.65}   & \DetailMed{8}         & \DetailAccMed{78.58}     & \DetailMed{8}     \\\DetailRaMedKeepSep
40   & \DetailAccMed{74.74}   & \DetailMed{9}         & \DetailAccMed{74.95}     & \DetailMed{10}     \\\DetailRaMedKeepSep
55   & \DetailAccMed{70.44}   & \DetailMed{10}        & \DetailAccMed{70.34}     & \DetailMed{11}     \\\DetailRaMedKeepSep
70   & \DetailAccMed{67.46}   & \DetailMed{9}         & \DetailAccMed{67.47}     & \DetailMed{11}     \\\DetailRaMedKeepSep
85   & \DetailAccMed{66.24}   & \DetailMed{10}        & \DetailAccMed{66.61}     & \DetailMed{12}     \\\DetailRaMedKeepSep
105  & \DetailAccMed{63.55}   & \DetailMed{10}        & \DetailAccMed{63.61}     & \DetailMed{12}     \\\DetailRaMedKeepSep
115  & \DetailAccMedB{62.39}  & \DetailMedB{11}       & \DetailAccMedTop{62.35}  & \DetailMedTop{13}     \\\DetailRaMedKeepSep
140  & \DetailAccMed{60.35}   & \DetailMed{10}        & \DetailAccMed{60.57}     & \DetailMed{12}     \\\DetailRaMedKeepSep
165  & \DetailAccMed{57.91}   & \DetailMed{8}         & \DetailAccMed{58.48}     & \DetailMed{10}     \\\DetailRaMedKeepSep
185  & \DetailAccMed{56.08}   & \DetailMed{7}         & \DetailAccMed{56.39}     & \DetailMed{9}     \\\DetailRaMedKeepSep
200  & \DetailAccMed{55.80}   & \DetailMed{7}         & \DetailAccMed{56.43}     & \DetailMed{9}     \\\DetailRaMedKeepSep
225  & \DetailAccMed{56.27}   & \DetailMed{6}         & \DetailAccMed{56.56}     & \DetailMed{8}     \\\DetailRaMedKeepSep
250  & \DetailAccMed{53.30}   & \DetailMed{4}         & \DetailAccMed{53.46}     & \DetailMed{5}     \\


==> tables/med-robust/detailed/ours/mnist.tex <==
     & \DetailAccHead{}       & \OursMedRobustHead{}  & \DetailAccHead{}         & \OursMedRobustHead{}     \\\midrule
5    & \DetailAccMed{99.50}   & \DetailMed{2}         & \DetailAccMed{99.51}     & \DetailMed{2}     \\\DetailRaMedKeepSep
10   & \DetailAccMed{98.64}   & \DetailMed{4}         & \DetailAccMed{98.67}     & \DetailMed{4}     \\\DetailRaMedKeepSep
15   & \DetailAccMed{96.82}   & \DetailMed{7}         & \DetailAccMed{97.02}     & \DetailMed{7}     \\\DetailRaMedKeepSep
20   & \DetailAccMed{96.36}   & \DetailMed{8}         & \DetailAccMed{96.53}     & \DetailMed{8}     \\\DetailRaMedKeepSep
25   & \DetailAccMedB{95.77}  & \DetailMedB{9}        & \DetailAccMed{96.06}     & \DetailMed{10}     \\\DetailRaMedKeepSep
35   & \DetailAccMed{91.70}   & \DetailMed{9}         & \DetailAccMed{93.05}     & \DetailMed{11}     \\\DetailRaMedKeepSep
40   & \DetailAccMed{89.37}   & \DetailMed{9}         & \DetailAccMed{91.32}     & \DetailMed{11}     \\\DetailRaMedKeepSep
50   & \DetailAccMed{84.54}   & \DetailMed{8}         & \DetailAccMed{88.46}     & \DetailMed{11}     \\\DetailRaMedKeepSep
60   & \DetailAccMed{83.54}   & \DetailMed{9}         & \DetailAccMedTop{87.22}  & \DetailMedTop{12}     \\\DetailRaMedKeepSep
70   & \DetailAccMed{79.71}   & \DetailMed{8}         & \DetailAccMed{85.87}     & \DetailMed{11}     \\\DetailRaMedKeepSep
80   & \DetailAccMed{71.29}   & \DetailMed{6}         & \DetailAccMed{79.05}     & \DetailMed{9}     \\\DetailRaMedKeepSep
90   & \DetailAccMed{69.94}   & \DetailMed{6}         & \DetailAccMed{79.25}     & \DetailMed{9}     \\\DetailRaMedKeepSep
105  & \DetailAccMed{62.53}   & \DetailMed{4}         & \DetailAccMed{74.45}     & \DetailMed{8}     \\\DetailRaMedKeepSep
120  & \DetailAccMed{63.03}   & \DetailMed{3}         & \DetailAccMed{74.09}     & \DetailMed{7}     \\\DetailRaMedKeepSep
130  & \DetailAccMed{57.48}   & \DetailMed{2}         & \DetailAccMed{69.93}     & \DetailMed{7}     \\\DetailRaMedKeepSep
150  & \DetailAccMed{52.51}   & \DetailMed{0}         & \DetailAccMed{67.30}     & \DetailMed{5}     \\


==> tables/med-robust/detailed/ours/weather.tex <==
     & \DetailAccHead{}         & \OursMedRobustHead{}        & \DetailAccHead{}       & \OursMedRobustHead{}     \\\midrule
1    & \DetailAccMed{92.70}     & \DetailMed{0}               & \DetailAccMed{86.05}   & \DetailMed{0}     \\\DetailRaMedKeepSep
5    & \DetailAccMed{85.29}     & \DetailMed{2}               & \DetailAccMed{83.34}   & \DetailMed{2}     \\\DetailRaMedKeepSep
11   & \DetailAccMed{82.48}     & \DetailMed{3}               & \DetailAccMed{79.55}   & \DetailMed{2}     \\\DetailRaMedKeepSep
15   & \DetailAccMed{81.09}     & \DetailMed{3}               & \DetailAccMedB{76.15}  & \DetailMedB{3}     \\\DetailRaMedKeepSep
21   & \DetailAccMedTop{76.10}  & \DetailMedTop{4}            & \DetailAccMed{67.09}   & \DetailMed{2}     \\\DetailRaMedKeepSep
25   & \DetailAccMed{71.40}     & \DetailMed{3}               & \DetailAccMed{64.77}   & \DetailMed{2}     \\\DetailRaMedKeepSep
31   & \DetailAccMed{67.06}     & \DetailMed{3}               & \DetailAccMed{58.71}   & \DetailMed{2}     \\\DetailRaMedKeepSep
35   & \DetailAccMed{62.56}     & \DetailMed{3}               & \DetailAccMed{55.95}   & \DetailMed{1}     \\\DetailRaMedKeepSep
41   & \DetailAccMed{60.19}     & \DetailMed{2}               & \DetailAccMed{51.57}   & \DetailMed{0}     \\\DetailRaMedKeepSep
51   & \DetailAccMed{55.34}     & \DetailMed{1}               & \DetailAccMed{45.84}   & \DetailMed{\DetailedNeg{}}     \\\DetailRaMedKeepSep
75   & \DetailAccMed{42.20}     & \DetailMed{\DetailedNeg{}}  & \DetailAccMed{26.93}   & \DetailMed{\DetailedNeg{}}     \\\DetailRaMedKeepSep
101  & \DetailAccMed{28.67}     & \DetailMed{\DetailedNeg{}}  & \DetailAccMed{21.26}   & \DetailMed{\DetailedNeg{}}     \\


==> tables/med-robust/detailed/ra/ames.tex <==
    & \DetailAccHead{}       & \RAMedRobustHead{}          & \DetailAccHead{}       & \RAMedRobustHead{}     \\\midrule
70  & \DetailAccMed{68.60}   & \DetailMed{0}               & \DetailAccMed{66.89}   & \DetailMed{0}     \\\DetailRaMedKeepSep
60  & \DetailAccMed{68.94}   & \DetailMed{0}               & \DetailAccMedB{67.24}  & \DetailMedB{1}     \\\DetailRaMedKeepSep
50  & \DetailAccMedB{67.58}  & \DetailMedB{1}              & \DetailAccMed{66.89}   & \DetailMed{1}     \\\DetailRaMedKeepSep
40  & \DetailAccMed{61.77}   & \DetailMed{1}               & \DetailAccMed{61.77}   & \DetailMed{1}     \\\DetailRaMedKeepSep
35  & \DetailAccMed{61.09}   & \DetailMed{0}               & \DetailAccMed{60.07}   & \DetailMed{1}     \\\DetailRaMedKeepSep
30  & \DetailAccMed{57.68}   & \DetailMed{0}               & \DetailAccMed{57.00}   & \DetailMed{1}     \\\DetailRaMedKeepSep
25  & \DetailAccMed{53.58}   & \DetailMed{0}               & \DetailAccMed{52.56}   & \DetailMed{1}     \\\DetailRaMedKeepSep
20  & \DetailAccMed{51.54}   & \DetailMed{0}               & \DetailAccMed{49.49}   & \DetailMed{\DetailedNeg{}}     \\\DetailRaMedKeepSep
15  & \DetailAccMed{45.05}   & \DetailMed{\DetailedNeg{}}  & \DetailAccMed{44.37}   & \DetailMed{\DetailedNeg{}}     \\\DetailRaMedKeepSep
10  & \DetailAccMed{37.20}   & \DetailMed{\DetailedNeg{}}  & \DetailAccMed{37.54}   & \DetailMed{\DetailedNeg{}}     \\\DetailRaMedKeepSep
5   & \DetailAccMed{33.79}   & \DetailMed{\DetailedNeg{}}  & \DetailAccMed{33.79}   & \DetailMed{\DetailedNeg{}}     \\


==> tables/med-robust/detailed/ra/cifar10.tex <==
     & \DetailAccHead{}       & \RAMedRobustHead{}  & \DetailAccHead{}       & \RAMedRobustHead{}     \\\midrule
250  & \DetailAccMed{88.77}   & \DetailMed{2}       & \DetailAccMed{88.56}   & \DetailMed{2}     \\\DetailRaMedKeepSep
225  & \DetailAccMed{88.05}   & \DetailMed{2}       & \DetailAccMed{87.90}   & \DetailMed{2}     \\\DetailRaMedKeepSep
200  & \DetailAccMed{86.76}   & \DetailMed{3}       & \DetailAccMed{86.54}   & \DetailMed{3}     \\\DetailRaMedKeepSep
175  & \DetailAccMed{86.16}   & \DetailMed{3}       & \DetailAccMed{85.94}   & \DetailMed{3}     \\\DetailRaMedKeepSep
150  & \DetailAccMed{84.23}   & \DetailMed{4}       & \DetailAccMed{84.08}   & \DetailMed{4}     \\\DetailRaMedKeepSep
125  & \DetailAccMed{82.66}   & \DetailMed{5}       & \DetailAccMed{82.49}   & \DetailMed{5}     \\\DetailRaMedKeepSep
100  & \DetailAccMed{80.43}   & \DetailMed{6}       & \DetailAccMed{80.05}   & \DetailMed{6}     \\\DetailRaMedKeepSep
75   & \DetailAccMedB{78.48}  & \DetailMedB{7}      & \DetailAccMed{78.11}   & \DetailMed{7}     \\\DetailRaMedKeepSep
50   & \DetailAccMed{73.26}   & \DetailMed{7}       & \DetailAccMed{72.79}   & \DetailMed{8}     \\\DetailRaMedKeepSep
35   & \DetailAccMed{70.34}   & \DetailMed{7}       & \DetailAccMed{69.72}   & \DetailMed{9}     \\\DetailRaMedKeepSep
30   & \DetailAccMed{69.62}   & \DetailMed{7}       & \DetailAccMed{69.01}   & \DetailMed{9}     \\\DetailRaMedKeepSep
25   & \DetailAccMed{68.81}   & \DetailMed{6}       & \DetailAccMed{68.08}   & \DetailMed{9}     \\\DetailRaMedKeepSep
20   & \DetailAccMed{67.01}   & \DetailMed{5}       & \DetailAccMed{66.15}   & \DetailMed{9}     \\\DetailRaMedKeepSep
15   & \DetailAccMed{65.68}   & \DetailMed{3}       & \DetailAccMedB{64.74}  & \DetailMedB{10}     \\\DetailRaMedKeepSep
12   & \DetailAccMed{63.93}   & \DetailMed{0}       & \DetailAccMed{62.91}   & \DetailMed{10}     \\\DetailRaMedKeepSep
10   & \DetailAccMed{62.73}   & \DetailMed{0}       & \DetailAccMed{61.71}   & \DetailMed{10}     \\\DetailRaMedKeepSep
8    & \DetailAccMed{60.24}   & \DetailMed{0}       & \DetailAccMed{59.12}   & \DetailMed{9}     \\\DetailRaMedKeepSep
7    & \DetailAccMed{59.08}   & \DetailMed{0}       & \DetailAccMed{57.83}   & \DetailMed{8}     \\\DetailRaMedKeepSep
5    & \DetailAccMed{53.20}   & \DetailMed{0}       & \DetailAccMed{51.84}   & \DetailMed{3}     \\


==> tables/med-robust/detailed/ra/mnist.tex <==
     & \DetailAccHead{}       & \RAMedRobustHead{}          & \DetailAccHead{}       & \RAMedRobustHead{}     \\\midrule
100  & \DetailAccMed{98.78}   & \DetailMed{4}               & \DetailAccMed{98.75}   & \DetailMed{4}     \\\DetailRaMedKeepSep
95   & \DetailAccMed{98.75}   & \DetailMed{5}               & \DetailAccMed{98.72}   & \DetailMed{5}     \\\DetailRaMedKeepSep
90   & \DetailAccMed{98.62}   & \DetailMed{5}               & \DetailAccMed{98.56}   & \DetailMed{5}     \\\DetailRaMedKeepSep
85   & \DetailAccMed{98.60}   & \DetailMed{5}               & \DetailAccMed{98.52}   & \DetailMed{5}     \\\DetailRaMedKeepSep
80   & \DetailAccMed{98.46}   & \DetailMed{6}               & \DetailAccMed{98.40}   & \DetailMed{6}     \\\DetailRaMedKeepSep
75   & \DetailAccMed{98.35}   & \DetailMed{6}               & \DetailAccMed{98.27}   & \DetailMed{6}     \\\DetailRaMedKeepSep
70   & \DetailAccMed{98.14}   & \DetailMed{6}               & \DetailAccMed{98.07}   & \DetailMed{6}     \\\DetailRaMedKeepSep
65   & \DetailAccMed{98.04}   & \DetailMed{7}               & \DetailAccMed{97.98}   & \DetailMed{7}     \\\DetailRaMedKeepSep
60   & \DetailAccMed{97.85}   & \DetailMed{7}               & \DetailAccMed{97.78}   & \DetailMed{7}     \\\DetailRaMedKeepSep
55   & \DetailAccMed{97.58}   & \DetailMed{7}               & \DetailAccMed{97.39}   & \DetailMed{8}     \\\DetailRaMedKeepSep
50   & \DetailAccMed{97.26}   & \DetailMed{7}               & \DetailAccMed{97.07}   & \DetailMed{8}     \\\DetailRaMedKeepSep
45   & \DetailAccMedB{96.88}  & \DetailMedB{8}              & \DetailAccMed{96.68}   & \DetailMed{8}     \\\DetailRaMedKeepSep
40   & \DetailAccMed{96.42}   & \DetailMed{8}               & \DetailAccMed{96.13}   & \DetailMed{9}     \\\DetailRaMedKeepSep
35   & \DetailAccMed{95.69}   & \DetailMed{8}               & \DetailAccMed{95.32}   & \DetailMed{9}     \\\DetailRaMedKeepSep
30   & \DetailAccMed{94.87}   & \DetailMed{7}               & \DetailAccMed{94.47}   & \DetailMed{9}     \\\DetailRaMedKeepSep
25   & \DetailAccMed{93.55}   & \DetailMed{6}               & \DetailAccMedB{93.09}  & \DetailMedB{10}     \\\DetailRaMedKeepSep
20   & \DetailAccMed{90.99}   & \DetailMed{3}               & \DetailAccMed{90.07}   & \DetailMed{9}     \\\DetailRaMedKeepSep
15   & \DetailAccMed{86.71}   & \DetailMed{0}               & \DetailAccMed{85.24}   & \DetailMed{8}     \\\DetailRaMedKeepSep
10   & \DetailAccMed{76.78}   & \DetailMed{0}               & \DetailAccMed{74.69}   & \DetailMed{6}     \\\DetailRaMedKeepSep
5    & \DetailAccMed{35.54}   & \DetailMed{\DetailedNeg{}}  & \DetailAccMed{32.89}   & \DetailMed{\DetailedNeg{}}     \\


==> tables/med-robust/detailed/ra/weather.tex <==
    & \DetailAccHead{}       & \RAMedRobustHead{}          & \DetailAccHead{}       & \RAMedRobustHead{}     \\\midrule
65  & \DetailAccMedB{80.70}  & \DetailMedB{0}              & \DetailAccMed{78.63}   & \DetailMed{0}     \\\DetailRaMedKeepSep
60  & \DetailAccMed{80.33}   & \DetailMed{0}               & \DetailAccMed{78.01}   & \DetailMed{0}     \\\DetailRaMedKeepSep
55  & \DetailAccMed{79.52}   & \DetailMed{0}               & \DetailAccMed{77.05}   & \DetailMed{0}     \\\DetailRaMedKeepSep
50  & \DetailAccMed{78.62}   & \DetailMed{0}               & \DetailAccMed{76.59}   & \DetailMed{0}     \\\DetailRaMedKeepSep
45  & \DetailAccMed{77.20}   & \DetailMed{0}               & \DetailAccMedB{75.19}  & \DetailMedB{1}     \\\DetailRaMedKeepSep
40  & \DetailAccMed{76.56}   & \DetailMed{0}               & \DetailAccMed{74.82}   & \DetailMed{1}     \\\DetailRaMedKeepSep
35  & \DetailAccMed{74.76}   & \DetailMed{0}               & \DetailAccMed{73.22}   & \DetailMed{1}     \\\DetailRaMedKeepSep
30  & \DetailAccMed{72.04}   & \DetailMed{0}               & \DetailAccMed{70.74}   & \DetailMed{1}     \\\DetailRaMedKeepSep
25  & \DetailAccMed{69.77}   & \DetailMed{0}               & \DetailAccMed{68.72}   & \DetailMed{1}     \\\DetailRaMedKeepSep
20  & \DetailAccMed{66.94}   & \DetailMed{0}               & \DetailAccMed{65.87}   & \DetailMed{1}     \\\DetailRaMedKeepSep
16  & \DetailAccMed{63.89}   & \DetailMed{0}               & \DetailAccMed{63.10}   & \DetailMed{1}     \\\DetailRaMedKeepSep
12  & \DetailAccMed{58.59}   & \DetailMed{0}               & \DetailAccMed{57.74}   & \DetailMed{1}     \\\DetailRaMedKeepSep
8   & \DetailAccMed{53.44}   & \DetailMed{0}               & \DetailAccMed{52.82}   & \DetailMed{0}     \\\DetailRaMedKeepSep
6   & \DetailAccMed{47.94}   & \DetailMed{\DetailedNeg{}}  & \DetailAccMed{47.25}   & \DetailMed{\DetailedNeg{}}     \\\DetailRaMedKeepSep
4   & \DetailAccMed{40.70}   & \DetailMed{\DetailedNeg{}}  & \DetailAccMed{39.91}   & \DetailMed{\DetailedNeg{}}     \\

